Dropout Injection at Test Time for Post Hoc Uncertainty Quantification in Neural Networks

Among Bayesian methods, Monte-Carlo dropout provides principled tools for evaluating the epistemic uncertainty of neural networks. Its popularity recently led to seminal works that proposed activating the dropout layers only during inference for evaluating uncertainty. This approach, which we call dropout injection, provides clear benefits over its traditional counterpart (which we call embedded dropout) since it allows one to obtain a post hoc uncertainty measure for any existing network previously trained without dropout, avoiding an additional, time-consuming training process. Unfortunately, no previous work compared injected and embedded dropout; therefore, we provide the first thorough investigation, focusing on regression problems. The main contribution of our work is to provide guidelines on the effective use of injected dropout so that it can be a practical alternative to the current use of embedded dropout. In particular, we show that its effectiveness strongly relies on a suitable scaling of the corresponding uncertainty measure, and we discuss the trade-off between negative log-likelihood and calibration error as a function of the scale factor. Experimental results on UCI data sets and crowd counting benchmarks support our claim that dropout injection can effectively behave as a competitive post hoc uncertainty quantification technique.

==> tables/dropout_activation.tex <==
\begin{table}
\caption{Differences between standard dropout used as a stochastic regularization technique~\cite{JMLR:v15:srivastava14a}, standard Monte-Carlo dropout used also for epistemic uncertainty evaluation~\cite{GalGahahr16} (embedded dropout) and Monte-Carlo dropout injection used only for epistemic uncertainty evaluation.
\label{tab:differences_dropout}}
{\begin{tabular}{lcc}
\hline
   & \begin{tabular}[c]{@{}c@{}}active at\\training time\end{tabular} & \begin{tabular}[c]{@{}c@{}}active at\\inference time\end{tabular}  \\ \hline
Standard dropout     & Yes     & No     \\ %\hline
(Embedded) Monte-Carlo dropout  & Yes     & Yes     \\ %\hline
Monte-Carlo dropout Injection   & No     & Yes     \\ \hline
\end{tabular}}{}
\end{table}
